$\rm \Lambda_{c}^{+}$ production and baryon-to-meson ratios in pp and p-Pb collisions at $\sqrt{s_\mathrm{NN}} = 5.02$ TeV at the LHC

The prompt production of the charm baryon $\rm \Lambda_{c}^{+}$ and the $\rm \Lambda_{c}^{+}/\mathrm {D^0}$ production ratios were measured at midrapidity with the ALICE detector in pp and p-Pb collisions at $\sqrt{s_\mathrm{NN}} = 5.02$TeV. These new measurements show a clear decrease of the $\rm \Lambda_{c}^{+}/\mathrm {D^0}$ ratio with increasing transverse momentum ($p_{\rm T}$) in both collision systems in the range $2<p_{\rm T}<12$ GeV/$c$, exhibiting similarities with the light-flavour baryon-to-meson ratios ${\rm p}/\pi$ and $\Lambda/\mathrm {K^0_S}$. At low $p_{\rm T}$, predictions that include additional colour-reconnection mechanisms beyond the leading-colour approximation; assume the existence of additional higher-mass charm-baryon states; or include hadronisation via coalescence can describe the data, while predictions driven by charm-quark fragmentation processes measured in $\mathrm {e^+e^-}$ and $\mathrm {e^-p}$ collisions significantly underestimate the data. The results presented in this letter provide significant evidence that the established assumption of universality (colliding-system independence) of parton-to-hadron fragmentation is not sufficient to describe charm-baryon production in hadronic collisions at LHC energies.

==> content/acknowledgements.tex <==


